Sample Complexity of Policy Gradient Finding Second-Order Stationary Points

The goal of policy-based reinforcement learning (RL) is to search the maximal point of its objective. However, due to the inherent non-concavity of its objective, convergence to a first-order stationary point (FOSP) can not guarantee the policy gradient methods finding a maximal point. A FOSP can be a minimal or even a saddle point, which is undesirable for RL. Fortunately, if all the saddle points are \emph{strict}, all the second-order stationary points (SOSP) are exactly equivalent to local maxima. Instead of FOSP, we consider SOSP as the convergence criteria to character the sample complexity of policy gradient. Our result shows that policy gradient converges to an $(\epsilon,\sqrt{\epsilon\chi})$-SOSP with probability at least $1-\widetilde{\mathcal{O}}(\delta)$ after the total cost of $\mathcal{O}\left(\dfrac{\epsilon^{-\frac{9}{2}}}{(1-\gamma)\sqrt\chi}\log\dfrac{1}{\delta}\right)$, where $\gamma\in(0,1)$. Our result improves the state-of-the-art result significantly where it requires $\mathcal{O}\left(\dfrac{\epsilon^{-9}\chi^{\frac{3}{2}}}{\delta}\log\dfrac{1}{\epsilon\chi}\right)$. Our analysis is based on the key idea that decomposes the parameter space $\mathbb{R}^p$ into three non-intersected regions: non-stationary point, saddle point, and local optimal region, then making a local improvement of the objective of RL in each region. This technique can be potentially generalized to extensive policy gradient methods.

==> macros.tex <==
%!TEX root = main.tex

\newcommand{\Thetabar}{\overline{\Theta}}

\newcommand{\eventcorcross}{\mathcal{E}^{\corRL,\mathrm{cross}}}
\newcommand{\Rtil}{\widetilde{R}}

\newcommand{\catelim}{\mathsf{CAT}\text{-}\mathsf{ELIM}}
\newcommand{\catvi}{\mathsf{CAT}}
\newcommand{\cat}{\mathsf{CAT}}

% Everything after this is non-italics
 \newtheorem{theorem}{Theorem}

\theoremstyle{definition} 
%Sets style of subsequent newtheorems to 'definition'
  \newtheorem{exercise}{Exercise}
  \newtheorem{claim}{Claim}[section]
  \newtheorem{lemma}[claim]{Lemma}
  \newtheorem{conjecture}{Conjecture}

\newtheorem{condition}{Condition}


  \newtheorem{informal}{Informal Theorem}


   \newtheorem{corollary}[theorem]{Corollary}
 \newtheorem{proposition}[theorem]{Proposition}
\newtheorem{example}{Example}
% Everything after this is italics
\theoremstyle{plain}
\newtheorem{remark}[claim]{Remark}

\newtheorem{definition}{Definition}[section]

\newcommand{\eventReg}{\calE^{\mathrm{reg}}}

\newcommand{\boldm}{\bm{m}}
\newcommand{\roundevent}{\mathcal{E}}
\newcommand{\qgreedy}{\qup\text{-greedy}}
\newcommand{\qgreedyk}{\qupk\text{-greedy}}
\newcommand{\dcoin}{\mathcal{D}^{\mathrm{coin}}}
\newcommand{\dcoink}{\dcoin_k}
\newcommand{\boldpiki}{\boldpik^{(i)}}
\newcommand{\boldpikboldik}{\boldpik^{(\boldi_k)}}
\newcommand{\pigreedksupi}{\pi^{\mathrm{grd},(i)}}
\newcommand{\boundbar}{\overline{\bound}}
\newcommand{\eventbonus}{\mathcal{E}^{\mathrm{bonus}}}
\newcommand{\eventratio}{\mathcal{E}^{\mathrm{rat}}}
\newcommand{\regretnom}{\mathrm{NominalRegret}}
\newcommand{\eventactiveset}{\mathcal{E}^{\activeset}}
\newcommand{\eventvi}{\mathcal{E}^{\mathrm{vi}}}
\newcommand{\rtilk}{\rtil_k}
\newcommand{\ptilk}{\ptil_k}
\newcommand{\eventcomp}{\mathcal{E}^{\mathrm{comp}}}
\newcommand{\boldi}{\boldsymbol{i}}
\newcommand{\supi}{^{(i)}}

\newcommand{\BigOh}[1]{{\mathcal{O}}\left(#1\right)}
\newcommand{\regret}{\mathrm{Reg}}
\newcommand{\epSet}{\mathcal{S}}
\newcommand{\type}{\mathsf{type}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\nSet}{N_{\epSet}}

\newcommand{\BigOhTil}[1]{\widetilde{\mathcal{O}}\left(#1\right)}
\newcommand{\LR}{\mathrm{LR}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calZ}{\mathcal{Z}}
\newcommand{\pl}{(1)}
\newcommand{\kl}{_{k,\ell}}
\newcommand{\klh}{_{k,\ell;h}}
\newcommand{\klpr}{_{k,\ell'}}
\newcommand{\klprh}{_{k,\ell';h}}
\numberwithin{equation}{section}
\newcommand{\vboldpi}{V^{\boldpi}}
\newcommand{\gapclip}{\ddot{\gap}}
\newcommand{\ck}{c_k}
\newcommand{\vpi}{\valf^{\pi}}
\newcommand{\nklsb}{N_{k,\ell;sb}}
\newcommand{\eventlocal}{\calE^{\mathrm{loc}}}
\newcommand{\bolddel}{\boldsymbol{\delta}}
\newcommand{\clsb}{C_{\ell;sb}}
\newcommand{\kH}{_{k;H}}
\newcommand{\xtil}{\widetilde{x}}
\newcommand{\eventcross}{\mathcal{E}^{\mathrm{err\,bound}}}
\newcommand{\eventsub}{\mathcal{E}^{\mathrm{sb}}}
\newcommand{\err}{\mathrm{Err}}
\newcommand{\errk}{\err_k}

\newcommand{\lsb}{_{\ell;sb}}

\newcommand{\klgl}{_{k,\ell;gl}}
\newcommand{\klsb}{_{k,\ell;sb}}
\newcommand{\wkl}{\weight\kl}
\newcommand{\wklh}{\weight\klh}
\newcommand{\nbar}{\overline{N}}
\newcommand{\nbark}{\nbar_k}
\newcommand{\chat}{\widehat{C}}
 \newcommand{\chatl}{\chat_{\ell,sb}}
\newcommand{\eventproblelst}{\mathcal{E}^{\mathrm{lead},\le\lst}}
\newcommand{\eventprobl}{\mathcal{E}^{\mathrm{lead},\ell}}
\newcommand{\Torus}{\mathbb{T}}
\newcommand{\astar}{a_{\star}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\klsttau}{_{k,\lst;\tau}}
\newcommand{\eventcorrlbonus}{\mathcal{E}^{\mathrm{bonus,CRANE}}}
\newcommand{\kappalelst}{\kappa_{\le\lst}}
\newcommand{\kappal}{\kappa_{\ell}}
\newcommand{\lbar}{\overline{\ell}}
\newcommand{\cbarl}{\cbar_{\ell}}
\newcommand{\eventvalconc}{\mathcal{E}^{\mathrm{val,conc}}}
\newcommand{\eventprobconc}{\mathcal{E}^{\mathrm{prb,conc}}}
\newcommand{\xaxpr}{(x,a,x')}
\newcommand{\goodeps}{\mathcal{K}_{\mathrm{good}}}
\newcommand{\advrange}{\adv^{\mathrm{range}}}
\newcommand{\corrupt}{\mathbf{C}}
\newcommand{\Errlead}{\mathrm{Err}^{\mathrm{val}}}
\newcommand{\klglb}{_{k,\ell,\mathrm{gl}}}
\newcommand{\klsub}{_{k,\ell,\mathrm{sb}}}
\newcommand{\klelst}{_{k,\le \lst}}
		\newcommand{\klst}{_{k,\lst}}

	\newcommand{\Pikl}{\Pi_{k}^{\ell}}
	\newcommand{\Piklelst}{\Pi_{k}^{\le\lst}}
\newcommand{\Pik}{\Pi_k}
\newcommand{\kli}{_{k,l,i}}
\newcommand{\klpl}{_{k,\ell+1}}
\newcommand{\klminh}{_{k,\ell-1;h}}
\newcommand{\piucb}[1]{\pi^{\mathrm{ucb},#1}}
\newcommand{\boldlk}{\boldl_k}
\newcommand{\Finite}[1]{\left[#1\right]_{<\infty}}
\newcommand{\nk}{N_k}
\newcommand{\nkl}{N_{k,\ell}}
\newcommand{\robustLfactor}{\Lfactor^{\mathrm{rbst}}}
\newcommand{\klih}{_{k,\ell,i;h}}
\newcommand{\Index}{\mathcal{I}}
		\newcommand{\klhpl}{_{k,\ell,h+1}}
\newcommand{\lfin}{\boldl^{\mathrm{fin}}}
\newcommand{\pik}{\pi_k}
\newcommand{\envir}{\mathscr{E}}
\newcommand{\boldpielim}{\boldpi^{\mathrm{unif}}}
\newcommand{\boldpielimk}{\boldpielim_k}
\newcommand{\lucbelim}{\mathsf{LUCBVI}\text{-}\mathsf{Elim}}
\newcommand{\Bernoulli}{\mathrm{Bernoulli}}
\newcommand{\False}{\mathsf{False}}
\newcommand{\True}{\mathsf{True}}
\newcommand{\isgreedy}{\mathsf{greedyAction}}
\newcommand{\Uniform}{\mathrm{Uniform}}
\newcommand{\plauset}{\activeset^{\mathrm{plaus}}}
\newcommand{\kHpl}{_{k;H+1}}
\newcommand{\kplh}{_{k+1;h}}
\newcommand{\fulelim}{\mathsf{FullElim}}
\newcommand{\xapr}{(x,a')}
\newcommand{\bonusk}{\bonus_k}
\newcommand{\lmax}{\ell^{\mathrm{max}}}
\newcommand{\klsth}{_{k,\lst;h}}
	\newcommand{\lst}{\ell_{\star}}
		\newcommand{\lkh}{\boldl\kh}
	
\newcommand{\Regret}{\mathrm{Regret}}

\newcommand{\pigreedboldl}{\pi^{\mathrm{grd},\,(\boldl)}}
	\newcommand{\pigreedboldlk}{\pi^{\mathrm{ucb},\,(\boldl)}_k}
	\newcommand{\pigreedboldlkk}{\pi^{\mathrm{ucb},\,(\boldl_k)}_k}
\newcommand{\distlayer}{\bm{\mathsf{P}}}

\newcommand{\boldpik}{\boldsymbol{\pi}_k}
\newcommand{\boldpil}{\boldsymbol{\pi}^{\ell}}
\newcommand{\boldpilk}{\boldsymbol{\pi}^{\ell}_k}

\newcommand{\boldpilel}{\boldsymbol{\pi}^{\le\ell)}}
\newcommand{\boldpilelst}{\boldsymbol{\pi}^{\le\lst}}


\newcommand{\boldpilelk}{\boldsymbol{\pi}^{\le\ell}_k}
\newcommand{\boldpilelstk}{\boldsymbol{\pi}^{\le\lst}_k}
\newcommand{\ellset}{\mathscr{L}}
\newcommand{\ellsetl}{\ellset_{\ell}}
\newcommand{\xkhakh}{(x\kh,a\kh)}

\newcommand{\klplh}{_{k,\ell+1;h}}
\newcommand{\oplustau}{\oplus_{\tau}}
\newcommand{\oplush}{\oplus_{h}}
\newcommand{\oplushbar}{\oplus_{\hbar}}
\newcommand{\vsthpl}{\vst_{h+1}}
\newcommand{\xah}{(x,a,h)}
\newcommand{\gap}{\mathrm{gap}}
\newcommand{\gapmin}{\gap_{\min}}
\newcommand{\clip}[2]{\operatorname{clip}\left[#2|#1\right]}
 \newcommand{\advhalfclip}{\dot{\adv}}
 \newcommand{\phatk}{\phat_k}
\newcommand{\rhatk}{\rhat_k}
\newcommand{\matE}{\mathbf{E}}

 \newcommand{\advlucbfullclip}{\ddot{\mathbf{E}}^{\mathrm{lucb}}}
 \newcommand{\advlucbhalfclip}{\dot{\mathbf{E}}^{\mathrm{lucb}}}
\newcommand{\advlucb}{\mathbf{E}^{\mathrm{lucb}}}


 \newcommand{\advfullclip}{\ddot{\adv}}
\newcommand{\gaph}{\mathrm{gap}_h}
\newcommand{\epsclip}{\epsilon_\mathrm{clip}}
\newcommand{\vsth}{\vst_h}
\newcommand{\mup}{\overline{\calM}}
\newcommand{\mlow}{\underline{\calM}}
\newcommand{\mlowk}{\mlow_k}
\newcommand{\mupk}{\mup_k}
\newcommand{\vupk}{\vup_k}
\newcommand{\vlowk}{\vlow_k}
\newcommand{\qlowk}{\qlow_k}
\newcommand{\qupk}{\qup_k}
\newcommand{\pigreedk}{\pigreed_k}
\newcommand{\ofx}{(x)}
\newcommand{\ofxh}{(x_h)}
\newcommand{\pisth}{\pist_{;h}}
\newcommand{\xhah}{(x_h,a_h)}
\newcommand{\optacts}{\mathcal{Z}_{opt}}
\newcommand{\subacts}{\mathcal{Z}_{sub}}
\newcommand{\nipsvspace}[1]{\iftoggle{nips}{\vspace{1}}{}}


\renewcommand{\ast}{a^\star}
\newcommand{\xast}{(x,\ast)}
\newcommand{\qsth}{\qst_h}
\newcommand{\bolda}{\mathbf{a}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\activeset}{\mathscr{A}}
\newcommand{\activesetk}{\activeset_k}
\newcommand{\tuple}{\mathscr{T}}
\newcommand{\tuplek}{\tuple_k}
\newcommand{\Kpl}{K^{\pl}}
\newcommand{\matz}{\mathbf{z}}
\newcommand{\matxpl}{\matx^{\pl}}
\newcommand{\matypl}{\maty^{\pl}}
\newcommand{\calEtil}{\widetilde{\mathcal{E}}}
\newcommand{\kclass}{\mathscr{K}}
\newcommand{\lossid}[1]{\mathcal{L}_{\mathrm{id},#1}}

\newcommand{\advlowgreed}{\advlow^{\mathrm{lcb}}}

\newcommand{\boldl}{\boldsymbol{\ell}}


\newcommand{\qf}{Q}
\newcommand{\vup}{\bar{\valf}}
\newcommand{\qup}{\bar{\qf}}
\newcommand{\qlow}{\makelow{\qf}}
\newcommand{\vlow}{\makelow{\valf}}

\newcommand{\valf}{V}
\newcommand{\vst}{\valf^{\star}}
\newcommand{\qst}{\qf^{\star}}
\newcommand{\pist}{\pi^{\star}}

\newcommand{\qcirc}{\mathring{\qf}}
\newcommand{\vcirc}{\mathring{\valf}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\adv}{\bar{\mathbf{E}}}

\newcommand{\advcirc}{\mathring{\adv}}

\newcommand{\occ}{\boldsymbol{\omega}}

\newcommand{\phat}{\widehat{p}}
\newcommand{\rhat}{\widehat{r}}

\newcommand{\rhatkhl}{\rhat_{k,h,\ell}}
\newcommand{\khl}{_{k;h;l}}
\newcommand{\khbar}{_{k;\hbar}}

\newcommand{\khboldl}{_{k;h,\boldl}}

\newcommand{\khlpr}{_{k;h,l'}}
\newcommand{\khpl}{_{k;h+1}}
\newcommand{\khpr}{_{k;h'}}

\newcommand{\khlh}{_{k;h,\boldl_h}}
\newcommand{\xa}{(x,a)}

\newcommand{\boundclipsah}{\tilde{\bound}}
\newcommand{\boundclip}{\check{\bound}}

\newcommand{\makelow}[1]{\mkern2mu\underline{\mkern-2mu#1\mkern-4mu}\mkern4mu }


\newcommand{\bonus}{\boldsymbol{b}}
\newcommand{\bonuskhl}{\bonus_{k,h,\ell}}
\newcommand{\bonusbar}{\overline{\bonus}}
\newcommand{\bonuscirc}{\mathring{\bonus}}

\newcommand{\nkhl}{n_{k,h,\ell}}
\newcommand{\Lfactor}{\mathbf{L}}
\newcommand{\Lcorrupt}{\mathbf{L}_{\mathrm{crpt}}}

\newcommand{\cbon}{c_{\bonus}}
\renewcommand{\hbar}{\tau}
\newcommand{\hboldbar}{\overline{\boldsymbol{\tau}}}

\newcommand{\Otilde}{\widetilde{O}}

\renewcommand{\ast}{a^\star}

\newcommand{\kh}{_{k;h}}
\newcommand{\ktau}{_{k;\tau}}

\newcommand{\kone}{_{k;1}}

\newcommand{\boldpi}{\boldsymbol{\pi}}
\newcommand{\pigreed}{\pi^{\mathrm{grd}}}
\newcommand{\piexp}{\pi^{\mathrm{exp}}}
\newcommand{\pimix}{\pi}
\newcommand{\pilcb}{\pi^{\mathrm{lcb}}}
\newcommand{\calMlow}{\makelow{\calM}}
\newcommand{\advlow}{\makelow{\mathbf{E}}}
\newcommand{\bonuslow}{\makelow{\bonus}\,}


\newcommand{\weight}{\boldsymbol{\omega}}
\newcommand{\weighthbar}{\weight^{\hbar}}

\newcommand{\khhbar}{_{k,h;\hbar}}
\newcommand{\khhboldbar}{_{k,h;\hboldbar}}
\newcommand{\dens}{\rho}
\renewcommand{\colon}{{\,:\,}}
\newcommand{\calM}{\mathcal{M}}

\newcommand{\calMbar}{\overline{\calM}}
\newcommand{\pbar}{\overline{p}}
\newcommand{\rbar}{\overline{r}}

\newcommand{\states}{\mathcal{X}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\outputs}{\mathcal{Y}}
\newcommand{\matx}{\mathbf{x}}
\newcommand{\mata}{\mathbf{a}}

\newcommand{\Gclass}{\mathscr{G}}
\newcommand{\Ust}{U_{\star}}
\newcommand{\Vst}{V_{\star}}
\newcommand{\sfP}{\mathsf{P}}

\newcommand{\Ast}{A_{\star}}
\newcommand{\Bst}{B_{\star}}
\newcommand{\Kst}{K_{\star}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\Khat}{\widehat{K}}
\newcommand{\matU}{\mathbf{U}}
\newcommand{\matDel}{\boldsymbol{\Delta}}
\newcommand{\Rhat}{\widehat{R}}

\newcommand{\Proj}{\mathrm{Proj}}
\newcommand{\ProjK}{\mathrm{Proj}_{\Kst}}
\newcommand{\ProjKzero}{\mathrm{Proj}_{\mathbf{0} \oplus \Kst}}
\newcommand{\veczero}{\mathbf{0}}

\newcommand{\Stief}{\mathrm{Stief}}
\newcommand{\nablabar}{\overline{\nabla}}
\newcommand{\nablacheck}{\check{\nabla}}
\newcommand{\fcheck}{\check{f}}
\newcommand{\Gcheck}{\check{G}}

\newcommand{\calK}{\mathcal{K}}
\newcommand{\calE}{\mathcal{E}}

\newcommand{\Rcheck}{\check{R}}

\newcommand{\xbar}{\overline{x}}
\newcommand{\xcheck}{\check{x}}

%comments

%ceiling

%theorems
{
 \theoremstyle{plain}
      \newtheorem{asm}{Assumption}
}
\newtheorem{nono-theorem}{Theorem}[]
\theoremstyle{plain}

\newtheorem{fact}[theorem]{Fact}
%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}
\newtheorem*{note}{Note}

\newtheorem{prop}[theorem]{Proposition}
\theoremstyle{definition}

\newtheorem{exc}{Exercise}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{obs}{Observation}[section]


%probability
\renewcommand{\Pr}{\mathbb{P}}
\newcommand{\Exp}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}

\newcommand{\Law}{\mathrm{Law}}
\newcommand{\Leb}{\mathrm{Lebesgue}}

\newcommand{\unifsim}{\overset{\mathrm{unif}}{\sim}}
\newcommand{\iidsim}{\overset{\mathrm{i.i.d.}}{\sim}}
\newcommand{\probto}{\overset{\mathrm{prob}}{\to}}
\newcommand{\ltwoto}{\overset{L_2}{\to}}

\newcommand{\info}{\mathbf{i}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\Ent}{\mathrm{Ent}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\rmd}{\mathrm{d}}

%math operators
\newcommand{\median}{\mathrm{Median}}
\newcommand{\range}{\mathrm{range}}
\newcommand{\im}{\mathrm{im }}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\spec}{\mathrm{spec}}
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\sign}{\mathrm{sign\ }}


%norms
\newcommand{\op}{\mathrm{op}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\dist}{\mathrm{dist}}

% logical
\renewcommand{\implies}{\text{ implies }}
\renewcommand{\iff}{\text{ iff }}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\matbeta}{\boldsymbol{\beta}}
\newcommand{\mattheta}{\boldsymbol{\theta}}

\newcommand{\betast}{\matbeta^*}
\newcommand{\betahat}{\widehat{\matbeta}}

\newcommand{\thetast}{\mattheta^*}
\newcommand{\thetahat}{\widehat{\mattheta}}
\newcommand{\supp}{\mathrm{supp}}


\newcommand{\matw}{\mathbf{w}}
\newcommand{\maty}{\mathbf{y}}


%Number Spaces
\renewcommand{\Im}{\mathfrak{Im }}
\renewcommand{\Re}{\mathfrak{Re }}

\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\C}{\mathbb{C}}

\newcommand{\I}{\mathbf{1}}
\newcommand{\Q}{\mathbb{Q}}

%Vector Spaces
\newcommand{\PD}{\mathbb{S}_{++}^d}
\newcommand{\sphered}{\mathcal{S}^{d-1}}




% Asymptotics

\newcommand{\BigThetaTil}[1]{\widetilde{\BigTm}\left({#1}\right)}
\newcommand{\BigOmega}[1]{\BigWm\left({#1}\right)}

\newcommand{\Rsimple}{\mathcal{R}_{\mathrm{simp}}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\actst}{a_*}
\newcommand{\acthat}{\widehat{a}}


\newcommand{\lasso}{\mathsf{lasso}}
\newcommand{\four}{\mathscr{F}}
\newcommand{\LS}{\mathsf{LS}}
\newcommand{\Alg}{\mathsf{Alg}}


\newcommand{\vi}{\matv^{(i)}}

% Complexity Classes
\newcommand{\SAT}{\mathit{SAT}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\NP}{\mathbf{NP}}
\newcommand{\coNP}{\co{NP}}
\newcommand{\co}[1]{\mathbf{co#1}}

\newcommand{\Drew}{\mathcal{D}_{\mathrm{rew}}}

\newcommand{\Drewtil}{\widetilde{\mathcal{D}}_{\mathrm{rew}}}
\newcommand{\ptil}{\widetilde{p}}
\newcommand{\rtil}{\widetilde{r}}
\newcommand{\calMtil}{\widetilde{\calM}}
\newcommand{\nomMDP}{{\calM}}
\newcommand{\didcorrupt}{c}
\newcommand{\matR}{\mathbf{R}}

\newcommand{\gapclipmin}{\ddot{\gap}_{\min}}

\newcommand{\ucb}{\mathrm{ucb}}
\newcommand{\lucb}{\mathrm{lucb}}
\newcommand{\lcb}{\mathrm{lcb}}
\newcommand{\aae}{\mathrm{aae}}

\newcommand{\boundlead}{\bound^{\mathrm{local}}}
\newcommand{\boundcross}{\bound^{\mathrm{cross}}}
\newcommand{\boundtotal}{\bound^{\mathrm{total}}}
\newcommand{\xau}{(x,a;u)}
\newcommand{\bound}{\mathbf{B}}

\newcommand{\cbar}{\overline{C}}
\newcommand{\scale}{scl}

\newcommand{\maxgap}{\check{\gap}}
%\newcommand{\boundclipsah}{\tilde{\bound}}
%\newcommand{\boundclip}{\check{\bound}}

%\newcommand{\I}{\mathbf{1}}


\newcommand{\corRL}{\mathsf{CRANE}\text{-}\mathsf{RL}}

\newcommand{\cL}{c_{\Lfactor}}
\newcommand{\Lf}{\Lfactor}

%%% macros for multi-layer stuff...
\newcommand{\pigreedboldllelst}{\boldpi^{\mathrm{grd},\,(\boldl_{\leq\lst})}}
  \newcommand{\pigreedboldlell}{\boldpi^{\mathrm{grd},\,(\boldl_{k,H} = \ell)}}
  \newcommand{\problesslst}{\mu(\mathcal{L}_{\leq \lst})}
  \newcommand{\probell}{\mu(\mathcal{L}_{\ell})}
  \newcommand{\klstgl}{_{k, \lst; gl}}
  \newcommand{\klsthpr}{_{k, \lst; h'}}
  \newcommand{\klhpr}{_{k,\ell; h'}}
  % \newcommand{\advlucbfullclip}{\ddot{\mathbf{E}}^{\mathrm{lucb}}}
% \newcommand{\advlucbhalfclip}{\dot{\mathbf{E}}^{\mathrm{lucb}}}
%\newcommand{\advlucb}{\mathbf{E}^{\mathrm{lucb}}}

 \newcommand{\wkih}{\weight_{k,i;h}}
  \newcommand{\wki}{\weight_{k,i}}
  \newcommand{\wti}{\weight_{t,i}}
  \newcommand{\Nsample}{N_{\mathrm{sample}}}
  \newcommand{\nbarki}{\nbar_{k,i}}
  \newcommand{\ki}{_{k,i}}
  \newcommand{\kih}{_{k,i,h}}
  \newcommand{\boundbari}{\boundbar\supi}
  \newcommand{\boundbarik}{\boundbari_k}
    \newcommand{\constc}{\alpha}
    \newcommand{\constcbar}{\bar{\constc}}
    \newcommand{\Mbar}{\bar{\constM}}
    \newcommand{\constM}{\beta}

  \newcommand{\nbari}{\nbar_{K,i}}

\newcommand{\nki}{N_{k,i}}

\newcommand{\boundk}{\bound_k}
\newcommand{\xtauatau}{(x_{\tau},a_{\tau})}
\newcommand{\wkh}{\weight\kh}
\newcommand{\wk}{\weight_k}
\newcommand{\eventsample}{\mathcal{E}^{\mathrm{sample}}}
\newcommand{\nbarK}{\nbar_K}


\newcommand{\eventktype}{\calE_{k,i}}

\newcommand{\coin}{\mathrm{coin}}
\newcommand{\Hkalg}{\calH_{k,\coin}}
\newcommand{\Hcoinatk}{\calH_{[k],\coin}}

\newcommand{\Hk}{\calH_{k}}
\newcommand{\Dcoink}{\mathcal{D}_{\coin,k}}
\newcommand{\episodeset}{\mathcal{S}}
\newcommand{\eptype}{\mathrm{type}}

\newcommand{\pitil}{\widetilde{\pi}}

\newcommand{\eventadm}{\calE^{\mathrm{adm}}} 
